New Lower Bounds in Merlin-Arthur Communication and Graph Streaming Verification

We show new lower bounds in the \emph{Merlin-Arthur} (MA) communication model and the related \emph{annotated streaming} or stream verification model. The MA communication model is an enhancement of the classical communication model, where in addition to the usual players Alice and Bob, there is an all-powerful but untrusted player Merlin who knows their inputs and tries to convince them about the output. Most functions have MA protocols with total communication significantly smaller than what would be needed without Merlin. We focus on the online MA (OMA) model, which is the MA analogue of one-way communication, and introduce the notion of \emph{non-trivial-OMA} complexity of a function. This is the minimum total communication needed by any non-trivial OMA protocol computing that function, where a trivial OMA protocol is one where Alice sends Bob roughly as many bits as she would have sent without Merlin. We prove a lower bound on the non-trivial-OMA complexity of a natural function \emph{Equals-Index} (basically the well-known Index problem on large domains) and identify it as a canonical problem for proving strong lower bounds on this complexity: reductions from it (i) reproduce and/or improve upon the lower bounds for all functions that were previously known to have large non-trivial-OMA complexity, (ii) exhibit the first explicit functions whose non-trivial-OMA complexity is superlinear, and even exponential, in their classical one-way complexity, and (iii) show functions on input size $n$ for which this complexity is as large as $n/\log n$. While exhibiting a function with $\omega(\sqrt{n})$ (standard) OMA complexity is a longstanding open problem, we did not even know of any function with $\omega(\sqrt{n})$ non-trivial-OMA complexity. We further extend the lower bounds to a related streaming model called annotated streaming.

==> LowerBound.tex <==






==> list_results.tex <==
\section{List of Results}

\subsection{Standard streaming}


\paragraph{Layering Lemma:}
	Let $G=(V,E)$ be a $k$-vertex-connected graph and let $t \in V$ be an arbitrary 
	vertex. There is a $[\Ot(kn),\Ot(n/k)]$ scheme which shows that there are $k$ 
	vertex-disjoint paths from $t$ to $v$ for all $v \in V-\set{t}$.


\paragraph{AM: Standard Stream}

\begin{enumerate}
	\item There is an $[\Ot(k n),\Ot(n/k)]$ scheme for vertex-connectivity using public randomness.
\end{enumerate}

\paragraph{MA: Standard Stream}

\begin{enumerate}
	\item There is an $[\Ot(k^2 n),\Ot(n)]$ scheme for vertex-connectivity using only private 
	randomness.
	\item There is an $[\Ot(k n),\Ot(n/k)]$ scheme for differentiating between $k$ and $2k$ 
	vertex-connectivity using only private randomness.	
\end{enumerate}

\subsection{Absolute Turnstile Streams}

The absolute turnstile model contains insertions and deletions of elements in $[n]$. After the 
stream, an element is ``present'' iff it has non-zero frequency (could be negative).
The promise is that the values of every coordinate are between $-\val$ and $\val$ at the end of the 
stream.

\begin{enumerate}
	\item We can prove strong lower bounds in this model
	\item Algorithms that are based on $L0$-samplers work in this model with only a $\polylog(n)$ 
	blow up in space. 
	\item This algorithm seems more natural than the XOR update model because we can think of the 
	stream as defining a weighted graph, and we are interested in the underlying undirected graph.
\end{enumerate}


\paragraph{$L0$-Samplers:}

\begin{problem}
	Given an absolute turnstile stream containing insertions and deletions of elements in $[n]$, output 
	an element whose frequency is non-zero. 
\end{problem}

\begin{enumerate}
	\item There is an algorithm that solves the above problem with probability $1-1/\poly(n) \cdot 
	\polylog(\val)$ using $O(\log \log \val \cdot \polylog(n))$ bits of space.
	\item Setting $\val = 2^{2^{\polylog(n)}}$ gives us a space bond of $\polylog(n)$ and a 
	success probability of $1-2^{-\polylog(n)}$.
	\item Algorithms based on L0 samplers work in this model (without any proof) with only a 
	$\polylog(n)$ blowup in 
	space for example spanning forest, edge connectivity, vertex connectivity, min-cut, cut sparsifiers 
	etc.
\end{enumerate}


\paragraph{Lower Bounds}

We get lower bounds in this model for connectivity and $k$-vertex connectivity.
Here $h$ is the proof size and $v$ is the verification space.

\begin{enumerate}
	\item Any $(h,v)$ scheme for connectivity satisfies the following: $(n \log \val +h) \cdot  v = 
	\Omega(n^2 \log \val)$.
	This means that if $h= O(n \log \val)$ then $v=\Omega(n)$. 
	There is also an algorithm that uses $\Ot(n)$ space without any proof.
	
	This lower bound also works for $k$-edge connectivity.
	
	\item Any $(h,v)$ scheme for $k$-vertex connectivity satisfies the following: $(\log \val +h) \cdot 
	v = \Omega(k n \log \val)$.
	This means that if $h= O(\log \val)$ then $v=\Omega(kn)$. 
	There is also an algorithm that uses $\Ot(kn)$ space without any proof.
	Finally, there is also an $[\Ot(n^2 \log \val),\Ot(1)]$ scheme
\end{enumerate}













==> sgt_ub.tex <==
\section{Classical Streaming Algorithms under SGT streams}

\subsection{Connectivity}

\subsection{Vertex Connectivity}

\subsection{Edge Connectivity}





